Converting the sub-Jovian desert of exoplanets to a savanna with TESS, PLATO and Ariel

There is a lack of exoplanets with sizes similar to Neptune orbiting their host stars with periods $\lesssim 3$ days -- hence the name ``sub-Jovian/Neptune desert''. Recently, several exoplanets have been confirmed to reside in the desert transforming it into a ``savanna'' with several ``giraffe'' planets (such as LTT 9779 b and TOI-674 b). The most prominent scenarios put forward for the explanation of the formation of the desert are related to the stellar irradiation destroying the primary atmosphere of certain specific exoplanets. We aim to present three targets (LTT 9779 b, TOI-674 b and WASP-156 b) which, when observed at wide wavelength ranges in infrared (IR), could prove the presence of these processes, and therefore improve the theories of planetary formation/evolution. We simulate and analyse realistic light curves of the selected exoplanets with PLATO/NCAM and the three narrow-band filters of Ariel (VISPhot, FGS1 and FGS2) based on TESS observations of these targets. We improved the precision of the transit parameters of the three considered planets from the TESS data. We find that the combination of the three narrow-band filters of Ariel can yield inner precision of $\lesssim 1.1\%$ for the planetary radii. Data from the three telescopes together will span decades, allowing the monitoring of changes in the planetary atmosphere through radius measurements. The three selected ``giraffe'' planets can be golden targets for Ariel, whereby the loss of planetary mass due to stellar irradiation could be studied with high precision, multi-wavelength (spectro-)photometry.

==> arielparams_table_old.tex <==
\begin{table*}
\caption{Derived transit parameters for LTT-9779 b, TOI-674 b and WASP-156 b from the three filters of Ariel and the combined values. The two parameters describing the noise, $\sigma_r$ and $\sigma_w$ can not be combined. In the case of WASP-156 b in the FGS2 band-pass, the red component of the correlated noise is consistent with $0$ ppm (i.e. the red noise is negligible).}
\label{tab:giraffes-ariel}
\centering
\begin{tabular}{l c c c c}
\hline
\hline
Parameter & VISPhot & FGS1 & FGS2 & Combined \\
\hline \\[\dimexpr-\normalbaselineskip+3pt]
\multicolumn{5}{c}{\textit{LTT 9779 b}} \\ [\dimexpr-\normalbaselineskip+12pt]
\hline
$a / R_S$ &  $3.796 \pm 0.045$ & $3.782 \pm 0.042$ & $3.771 \pm 0.051$ & $3.783 \pm 0.027$ \\ 
 $R_P / R_S$ &  $0.04470 \pm 0.00064$ & $0.04540 \pm 0.00060$ & $0.04561 \pm 0.00080$ & $0.04526 \pm 0.00040$ \\ 
 $b$ &  $0.9212 \pm 0.0022$ &  $0.9223 \pm 0.0020$ & $0.9231 \pm 0.0029$ & $0.9223 \pm 0.0014$ \\ 
 $P$ [days] &  $0.7920819 \pm 0.0000108$ & $0.7920699 \pm 0.0000092$ & $0.7920718 \pm 0.0000151$ & $0.7920744 \pm 0.0000069$ \\ 
 $t_C$ [days] & $-0.00025 \pm 0.00022$ & $-0.00010 \pm 0.00021$ & $-0.000039 \pm 0.00033$ & $-0.00012 \pm 0.00015$ \\ 
$\sigma_{r}$ [100 ppm] & $286 \pm 3$ & $278 \pm 3$ & $328 \pm 5$ & -- \\ $\sigma_{w}$ [100 ppm] & $2.954 \pm 0.016$ & $2.810 \pm 0.018$ & $3.952 \pm 0.024$ & --  \\ 
\hline
\\[\dimexpr-\normalbaselineskip+3pt]
\multicolumn{5}{c}{\textit{TOI-674 b}} \\ [\dimexpr-\normalbaselineskip+12pt]
\hline
$a / R_S$ &  $12.091 \pm 0.127$ & $12.158 \pm 0.085$ & $11.997 \pm 0.228$ & $12.125 \pm 0.092$ \\ 
 $R_P / R_S$ &  $0.11189 \pm 0.00050$ & $0.11177 \pm 0.00036$ & $0.10920 \pm 0.00186$ & $0.11175 \pm 0.00065$ \\ 
 $b$ &  $0.6700 \pm 0.0081$ &  $0.6651 \pm 0.0054$ & $0.6803 \pm 0.0137$ & $0.6679 \pm 0.0056$ \\ 
 $P$ [days] &  $1.9771524 \pm 0.0000087$ & $1.9771613 \pm 0.0000055$ & $1.9770939 \pm 0.0000373$ & $1.9771578 \pm 0.0000129$ \\ 
 $t_C$ [days] & $0.000127 \pm 0.00008$ & $0.000028 \pm 0.000049$ & $0.000673 \pm 0.000348$ & $0.000065 \pm 0.000120$ \\ 
$\sigma_{r}$ [100 ppm] & $304 \pm 10$ & $296 \pm 5$ & $2033 \pm 20$ & -- \\ 
$\sigma_{w}$ [100 ppm] & $8.119 \pm 0.042$ & $4.758 \pm 0.026$ & $21.051 \pm 0.130$ & --  \\ 
\hline
\\[\dimexpr-\normalbaselineskip+3pt]
\multicolumn{5}{c}{\textit{WASP-156 b}} \\ [\dimexpr-\normalbaselineskip+12pt]
\hline
$a / R_S$ &  $12.88 \pm 0.24$ & $13.05 \pm 0.21$ & $12.37 \pm 0.50$ & $12.93 \pm 0.20$ \\ 
 $R_P / R_S$ &  $0.06626 \pm 0.00045$ & $0.06677 \pm 0.00038$ & $0.06729 \pm 0.00103$ & $0.06661 \pm 0.00040$ \\ 
 $b$ &  $0.163 \pm 0.111$ &  $0.147 \pm 0.102$ & $0.303 \pm 0.125$ & $0.194 \pm 0.065$ \\ 
 $P$ [days] &  $3.836225 \pm 0.000058$ & $3.836049 \pm 0.000049$ & $3.836032 \pm 0.000090$ & $3.836110 \pm 0.000039$ \\ 
 $t_C$ [days] & $-0.000310 \pm 0.000230$ & $0.000430 \pm 0.000206$ & $0.000628 \pm 0.000415$ & $0.000160 \pm 0.000172$ \\ 
$\sigma_{r}$ [100 ppm] & $272 \pm 7$ & $295 \pm 6$ & $6 \pm 7$ & -- \\ 
$\sigma_{w}$ [100 ppm] & $7.563 \pm 0.026$ & $6.494 \pm 0.018$ & $13.156 \pm 0.052$ & --  \\ 
\hline
\end{tabular}
\end{table*}


==> binhex.tex <==
%%
%% This is file `binhex.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% binhex.dtx  (with options: `style')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from binhex.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file binhex.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\edef\next{\toks0=%
   {\catcode`\noexpand\@=\the\catcode`\@\toks0{\the\toks0}}%
}
\next
\catcode`\@11
\def\next#1#2#3{\expandafter \def \csname bb@#1\endcsname##1%
  {#2\csname bb@#3##1\endcsname}}
\next{00}00 \next{01}01 \next{02}10 \next{03}11
\next{04}20 \next{05}21 \next{06}30 \next{07}31
\next{08}40 \next{09}41 \next{10}50 \next{11}51
\next{12}60 \next{13}61 \next{14}70 \next{15}71
\next{16}80 \next{17}81 \next{18}90 \next{19}91
\expandafter \def \csname bb@0+\endcsname {+0}
\expandafter \def \csname bb@1+\endcsname {+1}
\def\bb@endbinary#1+{\fi\fi}
\expandafter \def \csname bb@0-\endcsname {0+-\bb@dobinary}
\expandafter\def\csname bb@0m\endcsname#1+{#1+0}
\expandafter\def\csname bb@1m\endcsname#1+{#1+1}
\def\bb@dobinary#1#2{\if#10\if m\string#2\else\bb@endbinary\fi\fi
 \expandafter\bb@dobinary\number\csname bb@0#1\endcsname#2}
\def\nbinary#1#2{\expandafter\bb@dobinary\number\number#2%
 \romannumeral\number\number#1 000+}
\def\binary{\nbinary1}
\def \next #1#2{\expandafter \def
 \csname bb@h\number +#1\endcsname ##1+{\bb@dohex ##1+#2}%
}
\next   {0}0 \next   {1}1 \next  {10}2 \next  {11}3
\next {100}4 \next {101}5 \next {110}6 \next {111}7
\next{1000}8 \next{1001}9 \next{1010}A \next{1011}B
\next{1100}C \next{1101}D \next{1110}E \next{1111}F
\def\bb@dohex #1{\csname bb@x#1\endcsname}
\def\bb@x\endcsname#1{ \bb@xm{m\endcsname}}
\def\bb@xm #1\endcsname #2#3+{#2#3%
 \csname bb@h\number+\endcsname
 #1\endcsname m#3+}
\def\bb@nbinbased #1#2#3{\expandafter \bb@dobinary \number#1%
 \expandafter \bb@dohex
 \romannumeral \number\number #2 000\expandafter\endcsname
 \romannumeral \number\number #3 000+}
\def\nbinbased #1#2#3{\expandafter\bb@nbinbased
 \expandafter {\number#3}{#2}{#1}}
\def\nhex{\nbinbased4}
\def\noct{\nbinbased3}
\def\ntetra{\nbinbased2}
\def\hex{\nhex1}
\def\oct{\noct1}
\def\tetra{\ntetra1}
\the\toks0
\endinput
%%
%% End of file `binhex.tex'.

